Design and Control of a Small Humanoid Equipped with Flight Unit and Wheels for Multimodal Locomotion

Humanoids are versatile robotic platforms owing to their limbs with multiple degrees of freedom. Although humanoids can walk like humans, they are relatively slow, and cannot run over large barriers. To address these limitations, we aim to achieve rapid terrestrial locomotion ability and simultaneously expand the locomotion domain to the air by utilizing thrust for propulsion. In this paper, we first describe an optimized construction method for a humanoid robot equipped with wheels and a flight unit to achieve these abilities. Then, we describe the integrated control framework of the proposed flying humanoid for each locomotion mode: aerial, legged, and wheeled locomotion. Finally, we achieved multimodal locomotion and aerial manipulation experiments using the proposed robot platform. To the best of our knowledge, this is the first time that a single humanoid has simultaneously achieved three different types of locomotion, including flight.

==> src/acknowledge.tex <==
\section*{ACKNOWLEDGMENT}

% The preferred spelling of the word acknowledgment in America is without an e after the g. Avoid the stilted expression, One of us (R. B. G.) thanks ...  Instead, try R. B. G. thanks. Put sponsor acknowledgments in the unnumbered footnote on the first page.

% References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.


